Revisiting Backdoor Attacks against Large Vision-Language Models from Domain Shift

Instruction tuning enhances large vision-language models (LVLMs) but increases their vulnerability to backdoor attacks due to their open design. Unlike prior studies in static settings, this paper explores backdoor attacks in LVLM instruction tuning across mismatched training and testing domains. We introduce a new evaluation dimension, backdoor domain generalization, to assess attack robustness under visual and text domain shifts. Our findings reveal two insights: (1) backdoor generalizability improves when distinctive trigger patterns are independent of specific data domains or model architectures, and (2) the competitive interaction between trigger patterns and clean semantic regions, where guiding the model to predict triggers enhances attack generalizability. Based on these insights, we propose a multimodal attribution backdoor attack (MABA) that injects domain-agnostic triggers into critical areas using attributional interpretation. Experiments with OpenFlamingo, Blip-2, and Otter show that MABA significantly boosts the attack success rate of generalization by 36.4%, achieving a 97% success rate at a 0.2% poisoning rate. This study reveals limitations in current evaluations and highlights how enhanced backdoor generalizability poses a security threat to LVLMs, even without test data access.

==> sections/4_Exploring_Attack_Scalability_against_LVLMs.tex <==

%\vspace{-0.2cm}
\section{Empirical Analysis with Domain Shift}

\subsection{Backdoor Attacks with Original Domain}
%\vspace{-0.1cm}
\label{sec:scalability}


This section evaluates the scalability of various attacks, specifically their effectiveness when applied from smaller models to LVLMs. We adhere to the parameters set by the backdoor attack benchmark \cite{backdoorbench, cui2022unified} and present the backdoor attack results for both visual and textual modalities.


\begin{figure}[ht]
\vspace{-0.cm}
\centering
\includegraphics[width=1.0\columnwidth]{images/img_lines.pdf}
\caption{Attack performance of different visual backdoor attacks with different poisoning rates and datasets.}
\label{fig:scalability}
% \vspace{-0.5cm}
\end{figure}

\textbf{Visual backdoor attack analysis.} Fig.~\ref{fig:scalability} depicts various backdoor attacks on input images, with poisoning rates on the horizontal axis and attack types differentiated by color. Solid lines show clean sample accuracy, while shaded areas indicate attack success rates (ASR). Key findings include: \ding{182} All visual backdoor attacks maintain high ASR (over 76.10\%) at 10\% poisoning rate, confirming scalability to LVLMs. \ding{183} WaNet and InputAware attacks underperform across poisoning rates in LVLMs due to their dependency on training adjustments, such as noise and contrast triggers requiring parameter tuning. \ding{184} Clean sample CIDEr scores in COCO are about 87\%, surpassing Openflamingo's 74\%, which motivates using microtuning sets to improve clean scores, adding further risks. \ding{185} Nonetheless, ASR remains consistently high across datasets (e.g., 97.62\% on COCO vs. 99.50\% on Flickr30K for Blended), showing robust triggering rates and performance despite dataset variations.

\begin{figure}[ht]
\vspace{-0.cm}
\centering
\includegraphics[width=1.0\columnwidth]{images/txt_lines.pdf}
\caption{Attack performance of different visual backdoor attacks with different poisoning rates and datasets.}
\label{fig:txt_scalability}
% \vspace{-0.5cm}
\end{figure}

\textbf{Textual backdoor attack analysis.} Tab.~\ref{tab:scalability} showcases results for textual backdoor attacks embedded in input questions at various poisoning rates, distinguished by color and aligned by character count. Key findings include: \ding{182} At high poisoning rates, most attacks succeed, but StyleBkd underperforms with an average character modification of 6.7, as its questions tranformed by text style blends compared slight difference with previous questions, reducing efficacy in large language models. \ding{183} Longer trigger patterns enhance attack success; for instance, at a 0.5\% poisoning rate, TextBadNets' ASR rises from 4.78\% with 6 characters to 54.38\% with 12 characters. Character-level attacks outperform sentence-level ones, with AddSent reaching a 51.28\% ASR at 0.5\% poisoning rate using 12 characters, while TextBadNets achieves 54.38\% under the same conditions. \ding{184} Triggers using special characters, like those in GCG, are highly effective, achieving over 99\% ASR at a 0.5\% poisoning rate with just 6 characters. This success is attributed to the rarity of special symbols in training, making them more conspicuous and easier to trigger.

\vspace{-0.1cm}
\begin{abox} % are we tired of takeaway boxes? :>
    \looseness -1 \textbf{Takeaways:} 1.~Attention sink emerges after LMs are trained on sufficient training data. 2.~Attention sink could be shifted to other positions rather than the first token if modifying $\color{cc2} p_{\textrm{data}}$.\looseness=-1% at test time.
\end{abox}



\section{Attack Generalizability on LVLMs}
\label{sec:generalizability}

% \subsection{Domain-Shifted Instruction Datasets}
\label{sec:construction}


% \textbf{Data construction pipeline}. To address challenges like task noise, instruction quality, and image duplication in constructing instruction sets deviating from the source domain, we employ a stable diffusion model and GPT-3.5 Turbo. We use the stable diffusion model to transform source domain images into two different art styles, Expressionism and Realism. For textual content, GPT-3.5 Turbo is used to summarize or expand questions and answers, adjusting information density while preserving original meanings. These transformations and additional details are documented in \emph{Supplementary Material}. The modified images and textual content are then recombined with the original instruction set elements to create six distinct instruction sets.



% \textbf{Statistical analysis.} We use the KS Statistic \cite{aguirre1998critique} to measure the distribution shift between original and generateed instruction domains, where a large KS Statistic indicates significant distribution differences. Initially, the open-source CLIP model calculates cosine similarities between images and text descriptions to establish a similarity distribution for each instruction set. We then compute the KS Statistic between the original and six modified instruction sets. Fig.~\ref{fig:statistics} illustrates the KS variation across different components of the instruction set, showing the largest variation in image distributions, followed by questions and then answers.


\begin{figure}[ht]
\centering
\includegraphics[width=0.95\columnwidth]{images/question-shift.pdf}
\caption{Attack performance and generalization when the textual question domain is shifted under MS COCO dataset.}
\label{fig:question}
% \vspace{-0.5cm}
\end{figure}

\subsection{Generalization with Question Domain Shift }
To assess the impact of input question domain variations on attack generalization, attackers used the Expansion Questio Shift and Summary Question Shift instruction sets as training sets, implanting text triggers at a 5\% poisoning rate. Fig.~\ref{fig:question} displays the ASR-G values of various text backdoor attack methods on the MS COCO dataset, where a value closer to 1 indicates better attack generalization. Key observations include: \ding{182} StyleBkd shows significant sensitivity to input domain changes, affecting its generalization due to its dependency on text domain reconstruction; \ding{183} Attack methods utilizing special characters, like GCG and $\text{GCG}^{*}$, demonstrate better generalization across text domain shifts, likely because these characters are less common in training data, maintaining high ASR across different domains. Additional results are available in the \emph{Supplementary Material.}.


\subsection{Generalization with Image Domain Shift }

\label{sec:image domain shift}
\input{tables/table2-image-domain}
To evaluate the impact of image domain variations on attack generalizability, we use a 5\% poisoning rate to balance attack performance and stealth. The attacker employs the Expressionism Image Shift and Realism Image Shift instruction sets as training sets, introducing poisoned samples. Attackers have access to the training process, allowing direct participation in model training, as seen with WaNet and DualKey attacks. The mean ASR-G represents the average ASR-G across two test sets.


% \text{Attack generalizability when the image domain is shifted}. As can be seen from the results in Tab.~\ref{tab:results}, changes in the image domain have a significant impact on the generalizability of the attack, usually exceeding the ability of the model itself to generalize to different domains. Specifically, we observe several key phenomena: \ding{182} A general decrease in attack generalization performance. While the performance of clean samples (\eg, CIDEr scores) decreases relative to the original instruction set, almost all attack algorithms also show a significant decrease in performance. This suggests that the bias of the image domain negatively affects the attack effectiveness more than it does the clean samples. \ding{183} Differences in image domain distribution have different impacts. Different styles of training image domains have varying effects on attack generalizability. For example, the Realism instruction set has a more severe negative impact on attack generalizability than the expressionist instruction set. For example, the Low Frequency method has a Mean ASR-G value of -0.99 in the Realism instruction set, compared to -0.27 in the Expressionism instruction set. This may be due to the greater distributional difference between the Realism instruction set and the original training data. \ding{184} The Case II attack method is the attack with the most severe decrease in generalizability. In particular, WaNet and Low Frequency methods perform extremely poorly on the realism instruction set, with Mean ASR-G -0.99, almost reaching the theoretical upper limit of the generalization performance degradation. This emphasizes that the generalization performance of the algorithms of the attack methods based on image characteristics is severely affected when the training data domain changes significantly.
\textbf{Attack generalizability when changing image domain.} Tab.~\ref{tab:image domain} shows that changes in the image domain significantly impact the generalizability of attacks. Key observations include: \ding{182} Generalization declines for most attacks; while clean samples (\eg, CIDEr scores) perform worse than the original instruction set, there is a notable drop in ASR across almost all attacks, indicating that image domain bias adversely affects attack effectiveness more than clean sample performance. \ding{183} The impact varies by image domain; the Realism instruction set substantially reduces attack generalizability more than the Expressionism set, with the Low Frequency attack yielding a Mean ASR-G of 0.01 for Realism versus 0.73 for Expressionism, likely due to greater distributional mismatch with the original training data. \ding{184} The Case II attack methods, especially WaNet and Low Frequency, show the most significant decline on the Realism set, with a Mean ASR-G as low as 0.01, highlighting severe generalization losses when there is a significant domain shift in training data.





% \textbf{Exceptional cases.} From Tab.~\ref{tab:results}, we observe that certain attack algorithms exhibit unusual generalization performance under specific conditions. \ding{182} The DualKey attack algorithm exhibits improved generalization performance in specific cases. This algorithm optimizes a trigger pattern that is semantically similar to the target based on the gradient information of the victim model. In particular, the generalization of the trigger patterns obtained by this algorithm is even improved under the expressivist instruction set, where the Mean ASR-G reaches 0.16. In contrast, when using the realist instruction set, DualKey's performance drops significantly, with a Mean ASR-G of -0.48. This suggests that the algorithm's generalization performance is significantly impacted by the choice of the training instruction set, although the the offset of the image domain can enhance the attack generalization in some cases, its stability is not sufficient. \ding{183} Stable generalization performance of Blended algorithm.Blended algorithm exhibits relatively stable attack generalization when the training data domain is varied. Its Mean ASR-G value basically stays near 0, indicating that the generalization of this attack method does not significantly decrease compared to the source domain. As an attack method that has little to do with image characteristics and model optimization, Blended maintains stable attack performance when the data domain changes significantly by virtue of its generalized triggering pattern.The success of the Blended attack inspires us that the Case I attack method shows promising prospects in terms of generalizability.
\textbf{Exceptional cases.} As seen in Tab.~\ref{tab:image domain}, certain attack algorithms demonstrate atypical generalization performance under specific conditions. \ding{182} The DualKey attack, which optimizes image triggers semantically equivalent to target text using the victim model's gradients, shows enhanced generalization in some scenarios. It excels under the Expressionist instruction set with a Mean ASR-G of 1 but struggles in the Realism set, achieving only a Mean ASR-G of 0.54. This suggests that the choice of training instruction set significantly influences the algorithm's generalization, highlighting how image domain shifts can both enhance and destabilize attack performance. \ding{183} The Blended attack exhibits the best generalization. Its Mean ASR-G remains stable at about 0.99, regardless of training data domain shifts. This attack maintains consistent performance across diverse data domains without significant impacts on picture attributes or model optimization, indicating that the Blended attack's generalized triggering mechanism may make it a broadly generalizable Case I attack method.



% \textbf{Attack generalization in combined image domains.} While the Blended algorithm shows good attack generalization in the cross-domain case, BadNets fails to perform well with image domain shifts, with Mean ASR-G of -0.90 and -0.82, respectively, which makes it impossible to generalize the generalization of Case I attack methods. In order to gain a deeper understanding of the reasons for BadNets' failure, we designed a series of experiments in which different ratios (20\%, 60\%, 80\%, 90\% and 98\%) of the constructed training instruction set were mixed with the original training instruction set to form a new training set for simulating image domain fusion. Fig.~\ref{} shows the attack results of the six attack algorithms with different mixing ratios. From Fig. x, we can conclude that \ding{182} Case I has good generalization performance. The generalization performance of the Case I attack method is excellent when the mixing ratio reaches 90\% and below. At this point, BadNets' generalization performance is comparable to Blended in all instruction domains. \ding{183} BadNets' generalization decreases. When the constructed training instruction set is dominant (more than 90\%), BadNets' generalization performance in the realism-style instruction set significantly decreases, especially in the 100\% constructed instruction set condition, where its performance fails completely. This suggests that BadNets' low generalization is not due to the trigger pattern itself, but rather to the fact that the triggers are too simple and easy to model learn and fail to adapt in the face of significant domain changes. We hypothesize that while the simplicity of BadNets' triggers allows the model to learn this pattern quickly in the domain of construction instructions, this simplicity also limits its adaptation in the original domain. When the domain changes significantly, especially in the case of 100\% constructed instruction sets, the model cannot effectively distinguish the difference between triggers and normal content. Thus, the low attack establishment rate is not due to the lack of generalization ability of the triggers themselves, but rather the failure of the learning process to adapt to the data characteristics of the original domain, leading to poor performance in the source domain.
% \begin{wrapfigure}{r}{0.6\textwidth}
%     \vspace{-20pt} % Adjust vertical space before the figure if needed
%     \centering
%     \includegraphics[width=0.59\textwidth, clip]{images/Domain_Percentage.pdf}
%     \caption{ASR of combined image domains with different proportions of attack algorithms.}
%     \label{fig:example}
%     \vspace{-10pt} % Adjust vertical space after the figure if needed
% \end{wrapfigure}
\begin{figure}[ht]
  \centering
  \begin{subfigure}{0.49\columnwidth}
    \includegraphics[width=\linewidth]{images/exp_ins.pdf}
    \caption{Expressionism Instruction}
    \label{fig:per_sub1}
  \end{subfigure}
  \begin{subfigure}{0.49\columnwidth}
    \includegraphics[width=\linewidth]{images/real_ins.pdf}
    \caption{Realism Instruction}
    \label{fig:per_sub2}
  \end{subfigure}
  \caption{ASR of combined image domains with different proportions of attack algorithms}
  \label{fig:percentage}  
\end{figure}


\begin{figure}[b]
\centering
\includegraphics[width=1.\columnwidth]{images/answer-shift.pdf}
\caption{Attack performance and generalization when the answer text domain is shifted under MS COCO dataset.}
\label{fig:answer statistics}
% \vspace{-0.5cm}
\end{figure}


\begin{figure*}[!t]
% \vspace{-0.7cm}
\centering
\includegraphics[width=0.9\textwidth]{images/Analysis_Method.pdf}
\caption{Analysis of the amount of change in Image-text correlation scores between clean and backdoor samples for different attacks.}
% \vspace{-0.3cm}
\label{fig:bar statistics}
\end{figure*}


\textbf{Attack generalization in combined image domains.} The Blended method exhibits robust attack generalization across domains, while BadNets significantly underperforms with Mean ASR-G values of 0.11 and 0.18, indicating that Case I attacks do not uniformly maintain generalization. To investigate this, we simulate image domain fusion by mixing 20\%, 60\%, 80\%, 90\%, and 98\% of a self-constructed instruction tuning set with the original set. Fig.~\ref{fig:percentage} displays the attack outcomes at various mixing ratios, leading to the following conclusions: \ding{182} BadNets maintains a high attack success rate with mixing ratios up to 90\%, suggesting its low generalization on self-constructed sets isn't due to trigger pattern flaws. Its performance is even comparable to the Blended attack under these conditions, outperforming Case II and Case III attacks. \ding{183} BadNets performs worse with a 90\% mixing ratio on the realism instruction set than with a 98\% ratio on the expressionism set, due to a greater distributional mismatch in the realism set. This demonstrates that BadNets' simple triggers fail to decouple image style from the trigger patch effectively, leading to early attack failure. Details of BadNets' CAM under cross-domain conditions are visualized in the \emph{Supplementary Material.}, revealing that while the trigger attracts attention, the model focuses more on other context, leading to attack failure.


\textbf{Image-model irrelevance is positively correlated with attack generalizability.} Image-model irrelevance refers to the independence of trigger pattern design from specific images or models. Case I trigger patterns, which do not rely on any particular picture or model, typically perform well across different image domains. Empirical analysis shows that these trigger patterns have a significant positive correlation with attack generalization performance. This indicates their ability to adapt to various domain changes and maintain effectiveness. It is worth emphasizing that it is also important to design appropriate triggers. If the trigger is too simple and the model does not learn enough, it may be affected by the contextual background information and lead to failure.




\subsection{Generalization with Answer Domain Shift }
% In order to assess the impact of changes in the text domain on the generalizability of the attack, the poisoning rate, the attack algorithm, the victimization model and the evaluation metrics align with the evaluation of changes in the image domain (Sec.~\ref{se}). In the experimental setup, the attacker implants malicious samples using the set of answer text abbreviations and amplified instructions as a training set and tests the attack generalizability on the COCO and Flickr datasets. The results of attacks in different text domains are shown in Tab.~\ref{tab:text domain}.
To evaluate the impact of text domain changes on attack generalizability, we use summary and expandish answer datasets as tuning sets. ASR and ASR\_origin represent attack outcomes in the shifted and original answer domains, respectively.

\textbf{Attack generalizability when changing answer domain}. Results from Fig.~\ref{fig:answer statistics} show that shifts in the answer domain positively impact attack generalizability. Key observations include: \ding{182} ASRs generally improve after training with offset answer domains, suggesting that these shifts do not significantly harm attack generalizability. \ding{183} Some attacks, like InputAware and DualKey, show varied generalizability across datasets, while StyleBkd proves ineffective. \ding{184} With textual answer domain offset, the COCO dataset of clean samples drops differently. This decline deserves to be greater since the Summary instruction dataset loses more textual details. However, this presumption is just the opposite in Fig.~\ref{fig:answer statistics}. This non-trivial phenomenon makes us ponder the attack success rate and clean sample performance trade-off.



% \input{tables/table_question_domain}
% As can be seen from the results on Tab.~\ref{tab:text domain}, the offset of the textual domain has a positive impact on the attack generalization property. We observe several key phenomena: \ding{182} The attack generalization performance of Case I and Case II remains almost the same or even improves. The generalization performance of Blended in Case I algorithm remains unchanged, and the Mean ASR-G of BadNets is also around 0, indicating that the change of textual training domain hardly affects the attack success rate. Second, the attack generalizability of Low Frequency and WaNet in the Case II algorithm improves with the change in the training text domain, with both Mean ASR-G exceeding 0, suggesting that the success rate of the attack now exceeds the success rate on the source domain. Although the distribution of the text domain is not shifted as drastically as that of the image domain, proper shifting has a reduced or even positive effect on the attack generalizability. \ding{183} Case III's attack algorithm performs erratically in terms of attack generalizability when the text domain is shifted.InputAware's attack success rate achieves an improvement in the Summary Instructions, but an Expansion Instructions, and the opposite is true for DualKey, which performs better in Expansion Instructions. This implies that the performance of these two attack algorithms related to model optimization is not stable for text domain shifts. The possible reason is that the change in textual domain directly affects the training process of the model by influencing the loss function.\ding{184} In the COCO dataset, the CIDEr of clean samples shows different degrees of decreases with the offset of the textual domain. In particular, this decrease is more pronounced due to the loss of more textual details in the Summary command. At this point, we also notice that the ASR-G is higher under the Summary instruction compared to the Expansion instruction. This non-trivial phenomenon led us to wonder whether there is some trade-off between attack success rate and clean sample performance.

\textbf{Image-text correlation analysis}. 
Offsets in the answer domain affect backdoor attack generalizability differently than those in the image domain, challenging the usual view that any training data offset is generally detrimental to model generalizability. We investigate extreme performances under Summary and Expansion Instructions: InputAware notably improves attack generalization with Summary Instructions, while StyleBkd attack generalization is ineffective; DualKey and WaNet show varied attack generalization improve under Expansion Instructions. To thoroughly examine these differences, we calculate the difference with the decrease in the image-text correlation score (total change is clean scores minus backdoor scores). Fig.~\ref{fig:bar statistics} indicates that for InputAware, DualKey and WaNet, the correlation scores decrease more for clean samples than for poisoned ones (Total Change Difference $>$ 0), suggesting that models respond more favorably to backdoor samples with answer domain offsets, thereby improving attack success rates. In contrast, StyleBkd shows a total change difference $<$ 0, indicating an increase in the prediction of clean samples but a decrease under poisoned conditions, thus causing attack failure. This implies a competitive dynamic between clean and poisoned samples in the decision-making process, where the reduced influence of clean samples bolsters the effects of poisoned samples, thus improving overall attack performance.

% The fact that offsets in the text domain have a very different impact on the generalizability of backdoor attacks than offsets in the image domain contradicts our usual understanding of model generalizability. It is generally accepted that any offset in the training data usually has a negative impact on the generalization performance of the model. Furthermore, we observe a trade-off between attack success and clean sample performance. To further explore how textual domain bias affects attack generalizability, we select the algorithms with the most extreme performance in the Summary Instructions and Expansion Instructions for analysis: in the Summary Instructions, InputAware (with a Mean ASR-G of 0.39) demonstrates the highest attack generalization enhancement, while WaNet (Mean ASR-G of 0.03) demonstrates the lowest; in Expansion Instructions, DualKey (Mean ASR-G of 0.16) and WaNet (Mean ASR-G of 0.01) exhibit different degrees of generalization, respectively.

% We analyze the original domain poisoned model and the textual domain poisoned model separately and calculate the correlation scores between clean and backdoor samples and their corresponding textual responses (\eg, descriptions related to ``banana''). In particular, we compared the amount of change in correlation scores between these samples in the original domain and the text domain, i.e., the change in correlation scores from the original domain poisoned model to the text domain poisoned model. The analysis showed that the decrease in correlation scores for clean samples (Clean Change) was generally higher than the decrease for poisoned samples (Poison change), for example, the amount of change in the expansion instructions was 4.79 for WaNet, 0.01 for the mean ASR-G, 94.15 for InputAware. Mean ASR-G of 0.39. This phenomenon suggests that the model is more inclined to respond to backdoor samples rather than clean samples in the face of textual domain offsets, which leads to an increase in the attack success rate. Therefore, we hypothesize that there is a competitive relationship between clean and poisoned samples in the model prediction decision-making process. A decrease in the influence of clean samples leads to a relative increase in the influence of poisoned samples, which is reflected in an overall increase in the attack success rate.

% \input{tables/Table6_Big_data}

\textbf{Preferred relevance is positively correlated with attack generalizability}. Trigger preferred relevance in backdoor attacks refers to how dominantly triggers influence model output. When poisoned sample triggers predominantly dictate the output, the model favors these malicious answers over the correct content. High trigger preferred relevance usually boosts attack generalizability, indicating that the model prefers responding to backdoor triggers even among conflicting signals from the original content. This principle supports the success of the Blended attack, which disrupts the clean sample's features, thus maintaining high generalizability. By diminishing the correlation between clean samples and correct responses, it becomes easier for the model to prioritize malicious commands over clean sample information.

\vspace{-0.1cm}
\begin{abox} % are we tired of takeaway boxes? :>
    \looseness -1 \textbf{Takeaways:} 1.~Attention sink emerges after LMs are trained on sufficient training data. 2.~Attention sink could be shifted to other positions rather than the first token if modifying $\color{cc2} p_{\textrm{data}}$.\looseness=-1% at test time.
\end{abox}



==> sections/5_Exploring_Attack_Generalizability_against_LVLMs.tex <==
% \section{Attack Generalizability on LVLMs}
% \label{sec:generalizability}

% % \subsection{Domain-Shifted Instruction Datasets}
% \label{sec:construction}


% % \textbf{Data construction pipeline}. To address challenges like task noise, instruction quality, and image duplication in constructing instruction sets deviating from the source domain, we employ a stable diffusion model and GPT-3.5 Turbo. We use the stable diffusion model to transform source domain images into two different art styles, Expressionism and Realism. For textual content, GPT-3.5 Turbo is used to summarize or expand questions and answers, adjusting information density while preserving original meanings. These transformations and additional details are documented in \emph{Supplementary Material}. The modified images and textual content are then recombined with the original instruction set elements to create six distinct instruction sets.



% % \textbf{Statistical analysis.} We use the KS Statistic \cite{aguirre1998critique} to measure the distribution shift between original and generateed instruction domains, where a large KS Statistic indicates significant distribution differences. Initially, the open-source CLIP model calculates cosine similarities between images and text descriptions to establish a similarity distribution for each instruction set. We then compute the KS Statistic between the original and six modified instruction sets. Fig.~\ref{fig:statistics} illustrates the KS variation across different components of the instruction set, showing the largest variation in image distributions, followed by questions and then answers.


% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.95\columnwidth]{images/question-shift.pdf}
% \caption{Attack performance and generalization when the textual question domain is shifted under MS COCO dataset.}
% \label{fig:question}
% % \vspace{-0.5cm}
% \end{figure}

% \subsection{Generalization with Question Domain Shift }
% To assess the impact of input question domain variations on attack generalization, attackers used the Expansion Questio Shift and Summary Question Shift instruction sets as training sets, implanting text triggers at a 5\% poisoning rate. Fig.~\ref{fig:question} displays the ASR-G values of various text backdoor attack methods on the MS COCO dataset, where a value closer to 1 indicates better attack generalization. Key observations include: \ding{182} StyleBkd shows significant sensitivity to input domain changes, affecting its generalization due to its dependency on text domain reconstruction; \ding{183} Attack methods utilizing special characters, like GCG and $\text{GCG}^{*}$, demonstrate better generalization across text domain shifts, likely because these characters are less common in training data, maintaining high ASR across different domains. Additional results are available in the \emph{Supplementary Material}.


% \subsection{Generalization with Image Domain Shift }

% \label{sec:image domain shift}
% \input{tables/table2-image-domain}
% To evaluate the impact of image domain variations on attack generalizability, we use a 5\% poisoning rate to balance attack performance and stealth. The attacker employs the Expressionism Image Shift and Realism Image Shift instruction sets as training sets, introducing poisoned samples. Attackers have access to the training process, allowing direct participation in model training, as seen with WaNet and DualKey attacks. The mean ASR-G represents the average ASR-G across two test sets.


% % \text{Attack generalizability when the image domain is shifted}. As can be seen from the results in Tab.~\ref{tab:results}, changes in the image domain have a significant impact on the generalizability of the attack, usually exceeding the ability of the model itself to generalize to different domains. Specifically, we observe several key phenomena: \ding{182} A general decrease in attack generalization performance. While the performance of clean samples (\eg, CIDEr scores) decreases relative to the original instruction set, almost all attack algorithms also show a significant decrease in performance. This suggests that the bias of the image domain negatively affects the attack effectiveness more than it does the clean samples. \ding{183} Differences in image domain distribution have different impacts. Different styles of training image domains have varying effects on attack generalizability. For example, the Realism instruction set has a more severe negative impact on attack generalizability than the expressionist instruction set. For example, the Low Frequency method has a Mean ASR-G value of -0.99 in the Realism instruction set, compared to -0.27 in the Expressionism instruction set. This may be due to the greater distributional difference between the Realism instruction set and the original training data. \ding{184} The Case II attack method is the attack with the most severe decrease in generalizability. In particular, WaNet and Low Frequency methods perform extremely poorly on the realism instruction set, with Mean ASR-G -0.99, almost reaching the theoretical upper limit of the generalization performance degradation. This emphasizes that the generalization performance of the algorithms of the attack methods based on image characteristics is severely affected when the training data domain changes significantly.
% \textbf{Attack generalizability when changing image domain.} Tab.~\ref{tab:image domain} shows that changes in the image domain significantly impact the generalizability of attacks. Key observations include: \ding{182} Generalization declines for most attacks; while clean samples (\eg, CIDEr scores) perform worse than the original instruction set, there is a notable drop in ASR across almost all attacks, indicating that image domain bias adversely affects attack effectiveness more than clean sample performance. \ding{183} The impact varies by image domain; the Realism instruction set substantially reduces attack generalizability more than the Expressionism set, with the Low Frequency attack yielding a Mean ASR-G of 0.01 for Realism versus 0.73 for Expressionism, likely due to greater distributional mismatch with the original training data. \ding{184} The Case II attack methods, especially WaNet and Low Frequency, show the most significant decline on the Realism set, with a Mean ASR-G as low as 0.01, highlighting severe generalization losses when there is a significant domain shift in training data.





% % \textbf{Exceptional cases.} From Tab.~\ref{tab:results}, we observe that certain attack algorithms exhibit unusual generalization performance under specific conditions. \ding{182} The DualKey attack algorithm exhibits improved generalization performance in specific cases. This algorithm optimizes a trigger pattern that is semantically similar to the target based on the gradient information of the victim model. In particular, the generalization of the trigger patterns obtained by this algorithm is even improved under the expressivist instruction set, where the Mean ASR-G reaches 0.16. In contrast, when using the realist instruction set, DualKey's performance drops significantly, with a Mean ASR-G of -0.48. This suggests that the algorithm's generalization performance is significantly impacted by the choice of the training instruction set, although the the offset of the image domain can enhance the attack generalization in some cases, its stability is not sufficient. \ding{183} Stable generalization performance of Blended algorithm.Blended algorithm exhibits relatively stable attack generalization when the training data domain is varied. Its Mean ASR-G value basically stays near 0, indicating that the generalization of this attack method does not significantly decrease compared to the source domain. As an attack method that has little to do with image characteristics and model optimization, Blended maintains stable attack performance when the data domain changes significantly by virtue of its generalized triggering pattern.The success of the Blended attack inspires us that the Case I attack method shows promising prospects in terms of generalizability.
% \textbf{Exceptional cases.} As seen in Tab.~\ref{tab:image domain}, certain attack algorithms demonstrate atypical generalization performance under specific conditions. \ding{182} The DualKey attack, which optimizes image triggers semantically equivalent to target text using the victim model's gradients, shows enhanced generalization in some scenarios. It excels under the Expressionist instruction set with a Mean ASR-G of 1 but struggles in the Realism set, achieving only a Mean ASR-G of 0.54. This suggests that the choice of training instruction set significantly influences the algorithm's generalization, highlighting how image domain shifts can both enhance and destabilize attack performance. \ding{183} The Blended attack exhibits the best generalization. Its Mean ASR-G remains stable at about 0.99, regardless of training data domain shifts. This attack maintains consistent performance across diverse data domains without significant impacts on picture attributes or model optimization, indicating that the Blended attack's generalized triggering mechanism may make it a broadly generalizable Case I attack method.



% % \textbf{Attack generalization in combined image domains.} While the Blended algorithm shows good attack generalization in the cross-domain case, BadNets fails to perform well with image domain shifts, with Mean ASR-G of -0.90 and -0.82, respectively, which makes it impossible to generalize the generalization of Case I attack methods. In order to gain a deeper understanding of the reasons for BadNets' failure, we designed a series of experiments in which different ratios (20\%, 60\%, 80\%, 90\% and 98\%) of the constructed training instruction set were mixed with the original training instruction set to form a new training set for simulating image domain fusion. Fig.~\ref{} shows the attack results of the six attack algorithms with different mixing ratios. From Fig. x, we can conclude that \ding{182} Case I has good generalization performance. The generalization performance of the Case I attack method is excellent when the mixing ratio reaches 90\% and below. At this point, BadNets' generalization performance is comparable to Blended in all instruction domains. \ding{183} BadNets' generalization decreases. When the constructed training instruction set is dominant (more than 90\%), BadNets' generalization performance in the realism-style instruction set significantly decreases, especially in the 100\% constructed instruction set condition, where its performance fails completely. This suggests that BadNets' low generalization is not due to the trigger pattern itself, but rather to the fact that the triggers are too simple and easy to model learn and fail to adapt in the face of significant domain changes. We hypothesize that while the simplicity of BadNets' triggers allows the model to learn this pattern quickly in the domain of construction instructions, this simplicity also limits its adaptation in the original domain. When the domain changes significantly, especially in the case of 100\% constructed instruction sets, the model cannot effectively distinguish the difference between triggers and normal content. Thus, the low attack establishment rate is not due to the lack of generalization ability of the triggers themselves, but rather the failure of the learning process to adapt to the data characteristics of the original domain, leading to poor performance in the source domain.
% % \begin{wrapfigure}{r}{0.6\textwidth}
% %     \vspace{-20pt} % Adjust vertical space before the figure if needed
% %     \centering
% %     \includegraphics[width=0.59\textwidth, clip]{images/Domain_Percentage.pdf}
% %     \caption{ASR of combined image domains with different proportions of attack algorithms.}
% %     \label{fig:example}
% %     \vspace{-10pt} % Adjust vertical space after the figure if needed
% % \end{wrapfigure}
% \begin{figure}[ht]
%   \centering
%   \begin{subfigure}{0.49\columnwidth}
%     \includegraphics[width=\linewidth]{images/Percentage_Expression.pdf}
%     \caption{Expressionism Instruction}
%     \label{fig:per_sub1}
%   \end{subfigure}
%   \begin{subfigure}{0.49\columnwidth}
%     \includegraphics[width=\linewidth]{images/Percentage_Realism.pdf}
%     \caption{Realism Instruction}
%     \label{fig:per_sub2}
%   \end{subfigure}
%   \caption{ASR of combined image domains with different proportions of attack algorithms}
%   \label{fig:percentage}  
% \end{figure}


% \begin{figure}[b]
% \centering
% \includegraphics[width=1.\columnwidth]{images/answer-shift.pdf}
% \caption{Attack performance and generalization when the answer text domain is shifted under MS COCO dataset.}
% \label{fig:answer statistics}
% % \vspace{-0.5cm}
% \end{figure}


% \begin{figure*}[!t]
% % \vspace{-0.7cm}
% \centering
% \includegraphics[width=0.9\textwidth]{images/Analysis_Method.pdf}
% \caption{Analysis of the amount of change in Image-text correlation scores between clean and backdoor samples for different attacks.}
% % \vspace{-0.3cm}
% \label{fig:bar statistics}
% \end{figure*}


% \textbf{Attack generalization in combined image domains.} The Blended method exhibits robust attack generalization across domains, while BadNets significantly underperforms with Mean ASR-G values of 0.11 and 0.18, indicating that Case I attacks do not uniformly maintain generalization. To investigate this, we simulate image domain fusion by mixing 20\%, 60\%, 80\%, 90\%, and 98\% of a self-constructed instruction tuning set with the original set. Fig.~\ref{fig:percentage} displays the attack outcomes at various mixing ratios, leading to the following conclusions: \ding{182} BadNets maintains a high attack success rate with mixing ratios up to 90\%, suggesting its low generalization on self-constructed sets isn't due to trigger pattern flaws. Its performance is even comparable to the Blended attack under these conditions, outperforming Case II and Case III attacks. \ding{183} BadNets performs worse with a 90\% mixing ratio on the realism instruction set than with a 98\% ratio on the expressionism set, due to a greater distributional mismatch in the realism set. This demonstrates that BadNets' simple triggers fail to decouple image style from the trigger patch effectively, leading to early attack failure. Details of BadNets' CAM under cross-domain conditions are visualized in the \emph{Supplementary Material}, revealing that while the trigger attracts attention, the model focuses more on other context, leading to attack failure.


% \textbf{Image-model irrelevance is positively correlated with attack generalizability.} Image-model irrelevance refers to the independence of trigger pattern design from specific images or models. Case I trigger patterns, which do not rely on any particular picture or model, typically perform well across different image domains. Empirical analysis shows that these trigger patterns have a significant positive correlation with attack generalization performance. This indicates their ability to adapt to various domain changes and maintain effectiveness. It is worth emphasizing that it is also important to design appropriate triggers. If the trigger is too simple and the model does not learn enough, it may be affected by the contextual background information and lead to failure.




% \subsection{Generalization with Answer Domain Shift }
% % In order to assess the impact of changes in the text domain on the generalizability of the attack, the poisoning rate, the attack algorithm, the victimization model and the evaluation metrics align with the evaluation of changes in the image domain (Sec.~\ref{se}). In the experimental setup, the attacker implants malicious samples using the set of answer text abbreviations and amplified instructions as a training set and tests the attack generalizability on the COCO and Flickr datasets. The results of attacks in different text domains are shown in Tab.~\ref{tab:text domain}.
% To evaluate the impact of text domain changes on attack generalizability, we use summary and expandish answer datasets as tuning sets. ASR and ASR\_origin represent attack outcomes in the shifted and original answer domains, respectively.

% \textbf{Attack generalizability when changing answer domain}. Results from Fig.~\ref{fig:answer statistics} show that shifts in the answer domain positively impact attack generalizability. Key observations include: \ding{182} ASRs generally improve after training with offset answer domains, suggesting that these shifts do not significantly harm attack generalizability. \ding{183} Some attacks, like InputAware and DualKey, show varied generalizability across datasets, while StyleBkd proves ineffective. \ding{184} With textual answer domain offset, the COCO dataset of clean samples drops differently. This decline deserves to be greater since the Summary instruction dataset loses more textual details. However, this presumption is just the opposite in Fig.~\ref{fig:answer statistics}. This non-trivial phenomenon makes us ponder the attack success rate and clean sample performance trade-off.



% % \input{tables/table_question_domain}
% % As can be seen from the results on Tab.~\ref{tab:text domain}, the offset of the textual domain has a positive impact on the attack generalization property. We observe several key phenomena: \ding{182} The attack generalization performance of Case I and Case II remains almost the same or even improves. The generalization performance of Blended in Case I algorithm remains unchanged, and the Mean ASR-G of BadNets is also around 0, indicating that the change of textual training domain hardly affects the attack success rate. Second, the attack generalizability of Low Frequency and WaNet in the Case II algorithm improves with the change in the training text domain, with both Mean ASR-G exceeding 0, suggesting that the success rate of the attack now exceeds the success rate on the source domain. Although the distribution of the text domain is not shifted as drastically as that of the image domain, proper shifting has a reduced or even positive effect on the attack generalizability. \ding{183} Case III's attack algorithm performs erratically in terms of attack generalizability when the text domain is shifted.InputAware's attack success rate achieves an improvement in the Summary Instructions, but an Expansion Instructions, and the opposite is true for DualKey, which performs better in Expansion Instructions. This implies that the performance of these two attack algorithms related to model optimization is not stable for text domain shifts. The possible reason is that the change in textual domain directly affects the training process of the model by influencing the loss function.\ding{184} In the COCO dataset, the CIDEr of clean samples shows different degrees of decreases with the offset of the textual domain. In particular, this decrease is more pronounced due to the loss of more textual details in the Summary command. At this point, we also notice that the ASR-G is higher under the Summary instruction compared to the Expansion instruction. This non-trivial phenomenon led us to wonder whether there is some trade-off between attack success rate and clean sample performance.

% \textbf{Image-text correlation analysis}. 
% Offsets in the answer domain affect backdoor attack generalizability differently than those in the image domain, challenging the usual view that any training data offset is generally detrimental to model generalizability. We investigate extreme performances under Summary and Expansion Instructions: InputAware notably improves attack generalization with Summary Instructions, while StyleBkd attack generalization is ineffective; DualKey and WaNet show varied attack generalization improve under Expansion Instructions. To thoroughly examine these differences, we calculate the difference with the decrease in the image-text correlation score (total change is clean scores minus backdoor scores). Fig.~\ref{fig:bar statistics} indicates that for InputAware, DualKey and WaNet, the correlation scores decrease more for clean samples than for poisoned ones (Total Change Difference $>$ 0), suggesting that models respond more favorably to backdoor samples with answer domain offsets, thereby improving attack success rates. In contrast, StyleBkd shows a total change difference $<$ 0, indicating an increase in the prediction of clean samples but a decrease under poisoned conditions, thus causing attack failure. This implies a competitive dynamic between clean and poisoned samples in the decision-making process, where the reduced influence of clean samples bolsters the effects of poisoned samples, thus improving overall attack performance.

% % The fact that offsets in the text domain have a very different impact on the generalizability of backdoor attacks than offsets in the image domain contradicts our usual understanding of model generalizability. It is generally accepted that any offset in the training data usually has a negative impact on the generalization performance of the model. Furthermore, we observe a trade-off between attack success and clean sample performance. To further explore how textual domain bias affects attack generalizability, we select the algorithms with the most extreme performance in the Summary Instructions and Expansion Instructions for analysis: in the Summary Instructions, InputAware (with a Mean ASR-G of 0.39) demonstrates the highest attack generalization enhancement, while WaNet (Mean ASR-G of 0.03) demonstrates the lowest; in Expansion Instructions, DualKey (Mean ASR-G of 0.16) and WaNet (Mean ASR-G of 0.01) exhibit different degrees of generalization, respectively.

% % We analyze the original domain poisoned model and the textual domain poisoned model separately and calculate the correlation scores between clean and backdoor samples and their corresponding textual responses (\eg, descriptions related to ``banana''). In particular, we compared the amount of change in correlation scores between these samples in the original domain and the text domain, i.e., the change in correlation scores from the original domain poisoned model to the text domain poisoned model. The analysis showed that the decrease in correlation scores for clean samples (Clean Change) was generally higher than the decrease for poisoned samples (Poison change), for example, the amount of change in the expansion instructions was 4.79 for WaNet, 0.01 for the mean ASR-G, 94.15 for InputAware. Mean ASR-G of 0.39. This phenomenon suggests that the model is more inclined to respond to backdoor samples rather than clean samples in the face of textual domain offsets, which leads to an increase in the attack success rate. Therefore, we hypothesize that there is a competitive relationship between clean and poisoned samples in the model prediction decision-making process. A decrease in the influence of clean samples leads to a relative increase in the influence of poisoned samples, which is reflected in an overall increase in the attack success rate.

% % \input{tables/Table6_Big_data}

% \textbf{Preferred relevance is positively correlated with attack generalizability}. Trigger preferred relevance in backdoor attacks refers to how dominantly triggers influence model output. When poisoned sample triggers predominantly dictate the output, the model favors these malicious answers over the correct content. High trigger preferred relevance usually boosts attack generalizability, indicating that the model prefers responding to backdoor triggers even among conflicting signals from the original content. This principle supports the success of the Blended attack, which disrupts the clean sample's features, thus maintaining high generalizability. By diminishing the correlation between clean samples and correct responses, it becomes easier for the model to prioritize malicious commands over clean sample information.

% \vspace{-0.1cm}
% \begin{abox} % are we tired of takeaway boxes? :>
%     \looseness -1 \textbf{Takeaways:} 1.~Attention sink emerges after LMs are trained on sufficient training data. 2.~Attention sink could be shifted to other positions rather than the first token if modifying $\color{cc2} p_{\textrm{data}}$.\looseness=-1% at test time.
% \end{abox}


==> tables/Tab_L.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
\multirow{3}{*}{Method} & \multirow{3}{*}{Type} & \multicolumn{7}{c}{ASR-G} \\
 &  & \multicolumn{3}{c}{Realism} & \multicolumn{3}{c}{Expressionism} & \multirow{2}{*}{mean} \\
 &  & OpenFlamingo & Otter & Blip-2 & OpenFlamingo & Otter & Blip-2 &  \\
Blended & Unimodal & 0.99 & 0.99 & 0.98 & 0.98 & 0.99 & 0.98 & 0.986 \\
BadNets & Unimodal & 0.13 & 0.15 & 0.94 & 0.18 & 0.19 & 0.01 & 0.318 \\
MABA & Unimodal & 0.81 & 0.82 & 0.21 & 0.77 & 0.8 & 0.26 & 0.682 \\
DualKey & Multimodal & 1 & 1 & 0.09 & 0.54 & 0.56 & 0.04 & 0.638 \\
MABA* & Multimodal 1 & 1 & 0.17 & 1 & 1 & 0.15 & 0.834
\end{tabular}%
}
\end{table}

==> tables/table1_PR_COCO.tex <==

\begin{table*}[ht]
    \centering
    \caption{Attack performance of different texual backdoor attacks with different poisoning rates in COCO dataset.}
    \label{tab:scalability}
    \resizebox{1\textwidth}{!}{%
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1}
    \begin{tabular}{lccccccccccc}
        \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Char Change} & \multicolumn{2}{c}{0.1\%} & \multicolumn{2}{c}{0.5\%} & \multicolumn{2}{c}{1\%} & \multicolumn{2}{c}{5\%} & \multicolumn{2}{c}{10\%} \\
        \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10} \cmidrule(r){11-12}
        & & ACC(\%) & ASR(\%) & ACC(\%) & ASR(\%) & ACC(\%) & ASR(\%) & ACC(\%) & ASR(\%) & ACC(\%) & ASR(\%) \\
        \midrule
        AddSent & 12 & 86.41 & 0.66 & 88.25 & 51.28 & 88.69 & 97.90 & 88.03 & 99.98 & 88.03 & 99.98 \\
        TextBadNets & 6 & 87.43 & 0.66 & 88.96 & 4.78 & 87.10 & 93.86 & 88.62 & 96.88 & 87.90 & 97.78 \\
        $\text{TextBadNets}^{*}$ & 12 & 86.25 & 0.68 & 86.96 & 54.38 & 87.41 & 98.78 & 88.23 & 99.94 & 88.06 & 99.96 \\
        StyleBkd & 6.7 & 87.15 & 0.00 & 83.99 & 0.00 & 86.87 & 29.64 & 88.94 & 25.20 & 86.88 & 29.64 \\
        GCG & 6 & 87.75 & 0.76 & 88.53 & 99.90 & 90.65 & 99.98 & 88.98 & 99.98 & 88.84 & 100.00 \\
        $\text{GCG}^{*}$ & 12 & 87.08 & 1.06 & 88.31 & 99.16 & 89.68 & 99.82 & 88.43 & 100.00 & 90.68 & 100.00 \\

        \bottomrule
    \end{tabular}%
    }
\end{table*}



==> tables/table3-text-domain.tex <==
\begin{table*}[h]
\vspace{-15pt}
    \centering
    \caption{Attack performance and generalization when the answer text domain is shifted.}
    \label{tab:text domain}
    \resizebox{0.95\textwidth}{!}{
        \begin{tabular}{lcccccccccccccc}
        \toprule
        \multirow{3}{*}{Method} & \multicolumn{7}{c}{Summary Answer Shift} & \multicolumn{7}{c}{Expansion Answer Shift} \\  
        \cmidrule(r){2-8} \cmidrule(r){9-15}
        & \multicolumn{3}{c}{COCO} & \multicolumn{3}{c}{Flickr30K} & \multirow{2}{*}{\shortstack{Mean \\ ASR-G}} & \multicolumn{3}{c}{COCO} & \multicolumn{3}{c}{Flickr30K} & \multirow{2}{*}{\shortstack{Mean \\ ASR-G}} \\
        \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){9-11} \cmidrule(r){12-14}
        & ACC & ASR & ASR-G & ACC & ASR & ASR-G & & ACC & ASR & ASR-G & ACC & ASR & ASR-G & \\
        \midrule
        BadNets & 80.94 & 98.68 & 0.99 & 45.39 & 99.7 & 1.00 & 1.00 & 86.27 & 94.82 & 0.95 & 45.72 & 99.1 & 0.99 & 0.97 \\
        Blended & 80.24 & 99.86 & 1.00 & 45.07 & 99.8 & 1.00 & 1.00 & 85.74 & 99.74 & 1.00 & 47.57 & 99.6 & 1.00 & 1.00 \\
        LowFrequency & 77.87 & 92.5 & 1.00 & 43.75 & 95.1 & 1.00 & 1.00 & 85.41 & 80.88 & 1.00 & 47.07 & 92.2 & 1.00 & 1.00 \\
        WaNet & 81.81 & 93.98 & 1.00 & 46.42 & 97.2 & 1.00 & 1.00 & 88.48 & 90.66 & 1.00 & 47.59 & 96.2 & 1.00 & 1.00 \\
        InputAware & 81.25 & 80.84 & 1.00 & 47.27 & 78.8 & 1.00 & 1.00 & 87.82 & 45.1 & 0.85 & 48.48 & 26.1 & 0.54 & 0.70 \\
        DualKey & 80.99 & 2.2 & 0.03 & 46.35 & 1.4 & 0.02 & 0.03 & 87.5 & 95.46 & 1.00 & 46.9 & 98.6 & 1.00 & 1.00 \\
        BadNetsx2 & 81.45 & 99.3 & 0.99 & 46.14 & 99 & 0.99 & 0.99 & 86.42 & 99.94 & 1.00 & 47.62 & 100 & 1.00 & 1.00 \\
        gcg & 81.08 & 99.9 & 1.00 & 45.81 & 100 & 1.00 & 1.00 & 88.1 & 99.94 & 1.00 & 48.13 & 100 & 1.00 & 1.00 \\
        gcgx2 & 80.89 & 100 & 1.00 & 46.73 & 100 & 1.00 & 1.00 & 88.29 & 99.66 & 1.00 & 48.55 & 100 & 1.00 & 1.00 \\
        addsent & 81.62 & 99.78 & 1.00 & 47.27 & 99.8 & 1.00 & 1.00 & 87.55 & 98.42 & 0.98 & 47.98 & 99.2 & 0.99 & 0.99 \\
        stylebkd & 74.32 & 4.7 & 0.19 & 43.9 & 0.49 & 0.02 & 0.10 & 86.31 & 4.7 & 0.19 & 46.18 & 4.9 & 0.19 & 0.19 \\
        \bottomrule
    \end{tabular}
   }
   \vspace{-0pt}
\end{table*}

==> tables/table_question_domain.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[h]
\caption{Attack performance and generalization when the question text domain is shifted.}
\centering
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{lcccccccccccccl}
\toprule
\multirow{3}{*}{Method} & \multicolumn{7}{c}{Summary Question Shift} & \multicolumn{7}{c}{Expansion Question Shift} \\ \cmidrule(r){2-8} \cmidrule(r){9-15}
 & \multicolumn{3}{c}{MSCOCO} & \multicolumn{3}{c}{Flickr} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Mean\\ ASR-G\end{tabular}} & \multicolumn{3}{c}{MSCOCO} & \multicolumn{3}{c}{Flickr} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Mean\\ ASR-G\end{tabular}}} \\ \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){9-11} \cmidrule(r){12-14}
 & ACC & ASR & ASR-G & ACC & ASR & ASR-G &  & ACC & ASR & ASR-G & ACC & ASR & ASR-G & \multicolumn{1}{c}{} \\ \midrule
badnets & 90.50 & 99.36 & 1.00 & 49.74 & 99.70 & 1.00 & 1.00 & 90.50 & 98.90 & 1.00 & 51.88 & 99.10 & 1.00 & 1.00 \\
BadNetsx2 & 90.81 & 99.86 & 1.00 & 50.12 & 100.00 & 1.00 & 1.00 & 91.96 & 99.50 & 1.00 & 52.53 & 99.70 & 1.00 & 1.00 \\
gcg & 92.38 & 100.00 & 1.00 & 50.76 & 100.00 & 1.00 & 1.00 & 91.36 & 99.82 & 1.00 & 50.22 & 100.00 & 1.00 & 1.00 \\
gcgx2 & 91.30 & 99.96 & 1.00 & 49.89 & 100.00 & 1.00 & 1.00 & 91.72 & 97.22 & 0.97 & 53.77 & 99.20 & 0.99 & 0.98 \\
addsent & 90.75 & 99.96 & 1.00 & 50.93 & 99.90 & 1.00 & 1.00 & 91.78 & 99.92 & 1.00 & 50.83 & 100.00 & 1.00 & 1.00 \\
stylebkd & 90.59 & 13.26 & 0.53 & 51.16 & 13.40 & 0.53 & 0.53 & 89.86 & 25.20 & 1.00 & 51.44 & 25.50 & 1.00 & 1.00 \\
\bottomrule
\end{tabular}%
}

\label{tab:my-table}
\end{table*}
